Evaluating Uncertainty-based Failure Detection for Closed-Loop LLM Planners

Recently, Large Language Models (LLMs) have witnessed remarkable performance as zero-shot task planners for robotic manipulation tasks. However, the open-loop nature of previous works makes LLM-based planning error-prone and fragile. On the other hand, failure detection approaches for closed-loop planning are often limited by task-specific heuristics or following an unrealistic assumption that the prediction is trustworthy all the time. As a general-purpose reasoning machine, LLMs or Multimodal Large Language Models (MLLMs) are promising for detecting failures. However, However, the appropriateness of the aforementioned assumption diminishes due to the notorious hullucination problem. In this work, we attempt to mitigate these issues by introducing a framework for closed-loop LLM-based planning called KnowLoop, backed by an uncertainty-based MLLMs failure detector, which is agnostic to any used MLLMs or LLMs. Specifically, we evaluate three different ways for quantifying the uncertainty of MLLMs, namely token probability, entropy, and self-explained confidence as primary metrics based on three carefully designed representative prompting strategies. With a self-collected dataset including various manipulation tasks and an LLM-based robot system, our experiments demonstrate that token probability and entropy are more reflective compared to self-explained confidence. By setting an appropriate threshold to filter out uncertain predictions and seek human help actively, the accuracy of failure detection can be significantly enhanced. This improvement boosts the effectiveness of closed-loop planning and the overall success rate of tasks.

==> chapter/failure_dataset.tex <==
\section{Calibration dataset}
% 

% To calibrate the uncertainty of the lava model, we collected one hundred twenty samples, including the states, during the execution of five tasks. The Realsense D415 collected these images.


For the LLaVA model, there is currently no evidence supporting the validity of employing token probability and entropy methods to obtain uncertainty. Valid uncertainty implies that higher model uncertainty correlates with decreased prediction accuracy. Conversely, as the model's confidence increases, its accuracy significantly improves. Additionally, the applicability of this uncertainty in robotic manipulation tasks remains uncertain. To investigate this, we collected 142 samples representing different execution states across five tasks\footnote{Task1:pick up the mouse and place it on the notebook, Task2:pick up the sponge and place it in the upper drawer, Task3:pick up the smartphone and place it on the drawer, Task4:open the upper drawer, Task5:close the upper drawer} \ref{calibration dataset}. The primary failures encompass detection and operational errors, explicitly excluding planning errors. The tasks primarily involve actions such as grasping, placing, and pushing. These images were captured using the Realsense D415 camera.
% 对于LLava模型，还没有任何证据可以证明使用token probability以及entropy方法获得的uncertainty是否合理，即当模型uncertainty较高时，其预测正确率较低，随着模型越来越自信，其正确率也明显提高，以及其uncertainty能否用于机器人实验，为了证明这一点，我们收集了120个样本，包含了五个任务的不同执行状态

\begin{table}[h]
\caption{calibration dataset break down}
\label{calibration dataset}
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
 & total &task 1 & task 2 & task 3 & task 4 & task 5\\
\hline
success & 72 & 12 & 18 & 12 & 18 & 12  \\
\hline
fail & 70 & 14 & 19 & 10 & 14 & 13  \\
\hline
\end{tabular}
\end{center}
\end{table}

% success & Four & 8 & 18 & 7 & 18 & 12  \\
% \hline
% fail & Four & 8 & 19 & 6 & 14 & 6  \\

==> chapter/introduction_old.tex <==
\section{INTRODUCTION}
% 1. 大语言模型正在被广泛的应用于机器人操作任务中，由于大语言强大的语言能力一起较为完善的常识知识，它能够将人类语言指令所指示的长期任务转换成多个短期任务，或者根据当前状态进行技能选择
% 2. 使用大语言模型进行任务规划的方式主要有两种，一种是开环控制，在完成任务规划后，机器人将一直按照初始的规划进行动作执行，另一种是闭环控制，当大语言模型最初生成的任务规划并非最优时，可以根据当前的环境反馈不断的调整规划和动作，以达到最终的目的
% 3. 在闭环规划中有一个很重要的环节便是如何根据当前环境的反馈，判断先前的动作或者任务是否执行成功，或者当前状态下，是否需要更新任务规划，在大部分当前的闭环控制算法中，（inner monologe）是人为的指定了一个检测函数，用于检测物体是否被抓取成功，（adaplanner）则是通过仿真系统返回的文字描述，传给大语言模型后尤其判断是否要重新规划
% 4. 损失函数检测的方法的局限性很强，只能用于特定的任务检测。由大语言模型独自进行判断时，由于语言模型缺少对于物理世界的认知，并且存在hallucination的可能，其判断结果的准确率较低，并且可能出现hallucination的情况，对于判断结果over confident.
% 5. 为了减少大语言模型在判断时出现over confident的情况，我们提出了将大语言模型confidence 量化的方法，通过量化标准对判断结果进行校正，在大语言模型无法进行准确判断时，请求人类反馈进行协助
Large language models (LLMs) are increasingly utilized in robotic manipulation tasks, acting as task planning and decision-making agents. Unlike robot learning approaches such as imitation learning (IL) and reinforcement learning (RL), which rely on expert demonstrations or direct environmental interactions, LLMs benefit from pre-training on vast, diverse textual datasets. 
This endows them with extensive worldly knowledge and reasoning capabilities. 
Consequently, LLMs can function as zero-shot planners, adeptly breaking down complex, long-term tasks into manageable, short-term objectives \cite{pmlr-v162-huang22a}.

Furthermore, LLMs facilitate natural language communication, streamlining human-robot interactions. 
This not only enhances collaborative efforts but also empowers non-experts to modify or rectify robot actions easily.

Recent initiatives \cite{ahn2022i} \cite{driess2023palme} have explored utilizing LLMs as planners with pre-trained skill libraries for real-world interactions. 
Nevertheless, this approach necessitates substantial data for skill library development. 
In response, works such as those by Huang et al. \cite{huang2023voxposer} and Liang et al. \cite{liang2023code} leverage LLMs' advanced programming skills, coupled with voxel map-derived physical data to translate necessary actions into executable Python code for robots.

% Nowadays, some works have already tried to leverage LLMs as planners and rely on a pre-trained skill library to interact with the real world. However, this type of method requires a large amount of data for training the skill library. To address this issue, \cite{huang2023voxposer} and \cite{liang2023code} leverages the powerful programming capabilities of LLMs, combined with the physical information obtained from the voxel map, to convert the required actions into Python code, which can be directly executed by the robot.

Current strategies predominantly employ open-loop control, rigidly following initial plans without incorporating environmental feedback. Consequently, execution errors or plan deficiencies remain unaddressed, potentially leading to task failure. To overcome these limitations, new models incorporating closed-loop control have been proposed. These models utilize LLMs, Vision Language Models (VLMs), or specific loss functions for anomaly detection, recalibrating the plan based on detected discrepancies \cite{sun2023adaplanner}, \cite{liu2023reflect}.

Although loss function-based anomaly detection is relatively accurate, its rigidity limits application to specific tasks. On the other hand, detection accuracy via LLMs or VLMs is compromised by the nascent state of multimodal models, often leading to hallucinations and overconfidence issues.

To improve the reliability of visual detections in multimodal models, this paper advocates for applying uncertainty quantification methods. By calibrating detection results, we aim to mitigate model hallucinations and enhance closed-loop control effectiveness in robotic manipulation, thereby boosting task success rates.
The contributions made in this work are as follows:
\begin{itemize}
    \item 
    \item 
    \item 
\end{itemize}
% However, these algorithms are all based on open-loop control. They will only execute actions according to the initial plan to complete the task and do not receive feedback from the environment. If errors occur during execution or if the plan itself has flaws, they will not correct them, thus leading to task failure.
% To address this issue, \cite{sun2023adaplanner}, \cite{liu2023reflect} proposed large language model planners capable of closed-loop control. They utilize LLM, VLM, or specific loss functions for anomaly detection. When anomalies are detected, the LLM is invoked again to analyze the errors and update the plan accordingly.
% The accuracy of anomaly detection using the loss function is relatively high, but the method is not sufficiently flexible and can only be applied to specific tasks. When using LLM or VLM, due to the immaturity of the current multimodal model, the accuracy of detection is lower. Language models often experience hallucinations and overconfidence.

% To enhance the reliability of the visual detection results of multimodal models, we propose utilizing uncertainty quantification methods to calibrate the detection outcomes, reducing model hallucination phenomena, and applying them to closed-loop control in robot manipulation tasks, thereby improving task completion rates.
\TODO{TODO: Add Teaser Figure and System Sketch Figure!}
